Differential Modulation and Non-Coherent Detection in Wireless Relay Networks

The technique of cooperative communications is finding its way in the next generations of many wireless communication applications. Due to the distributed nature of cooperative networks, acquiring fading channels information for coherent detection is more challenging than in the traditional point-to-point communications. To bypass the requirement of channel information, differential modulation together with non-coherent detection can be deployed. This thesis is concerned with various issues related to differential modulation and non-coherent detection in cooperative networks. Specifically, the thesis examines the behaviour and robustness of non-coherent detection in mobile environments (i.e., time-varying channels). The amount of channel variation is related to the normalized Doppler shift which is a function of user's mobility. The Doppler shift is used to distinguish between slow time-varying (slow-fading) and rapid time-varying (fast-fading) channels. The performance of several important relay topologies, including single-branch and multi-branch dual-hop relaying with/without a direct link that employ amplify-and-forward relaying and two-symbol non-coherent detection, is analyzed. For this purpose, a time-series model is developed for characterizing the time-varying nature of the cascaded channel encountered in amplify-and-forward relaying.

==> sections/acknowledge.tex <==
\chapter*{Acknowledgements}
Stephan Hawking, in his book: The Grand Design, ingeniously kids that: ``The universe has a design, and so does a book. But unlike the universe, a book does not appear spontaneously from nothing." I guess this argument applies to any kind of work no matter how valuable it would be and so does my thesis. In conducting the research and preparing this dissertation I have been blessed with the the help, inspiration and motivation of many people that I may not remember all of them. 
 
First and foremost, I would like to express my deepest gratitude toward my supervisor, Professor Ha H. Nguyen, for his criticism, patience, invaluable support and guidance throughout my research program at the University of Saskatchewan. It has truly been my honour and rewarding experience to work under his supervision. I have learnt several important lessons on the skills and values of conducting research.

I would also like to extend my gratitude to Professors Reza Fotouhi, Aryan S. Saadat-
Mehr, Francis Bui from the University of Saskatchewan, and Professor Alagan Anpalagan from Ryerson University, for serving in my doctoral committee. Their insightful advice and comments have improved the quality of this thesis.

My deepest love and gratitude go to my family for their unconditional love, care
and support for each and every endeavour in my life. I would also like to thank all my past and current members of our research group and my friends for the wonderful time we had together. I have enjoyed many discussions with them on various technical and non-technical topics.

This dissertation is dedicated to:
``Those who live, are those who strive, those whose
soul, possessed of a firm design, whose mind
envisioning a great destiny and a demanding climb,
walk pensive, engrossed by a goal sublime"
Victor Hugo


==> sections/chapter3.tex <==
\chapter{Completed Work}
\label{ch-completed}
As stated earlier, the objective of this research is to study non-coherent differential modulation and demodulation for relay networks to avoid any channel estimation. We aim to consider both slow-fading and time-varying channels. In this chapter, four main contributions obtained so far are summarized. In the first completed part \cite{DAF-SC}, a selection combiner is introduced for a three-node D-AF network and its performance is derived analytically and compared with MRC method. In the second and third completed parts \cite{DAF-WCNC,DAF-ITVT} we study D-AF with three and multi-node in time-varying Rayleigh fading channels. In the last work \cite{DH-CWIT}, a dual-hop network is studied in time-varying channels and a multiple-symbol differential detection is developed to improve its performance.


\section{Selection Combining for D-AF Relaying Over Rayleigh-Fading Channels}

In this work, we study a three-node relay network with one source, one relay and one destination. Differential $M$PSK (D$M$PSK) is used at the source to encode the information. The relay utilizes AF protocol with a fixed gain. At the destination, the decision variable is computed for each link and the one with the maximum magnitude is chosen for non-coherent detection. Hence, different from the MRC technique, the selection combiner does not need the second-order statistic of any of the channels, which simplifies the destination's
detection task. The probability density function (pdf) and commutative density function (cdf) of the instantaneous signal to noise ratio (SNR) in each link and the combiner's output are derived and used to obtain the exact average bit-error-rate (BER) and the outage probability of the system. It is shown that the desired diversity can be achieved. In addition, the BER expression is evaluated for optimum power allocation between the source and the relay. It is seen that more power should be allocated to the source than the relay in general and BER will be minimized if $70\%$ of the total power is allocated to the source and the rest to the relay. The analysis is verified with simulation. Comparison of SC and MRC systems shows that the performance of SC is very close to that of the MRC, of course with a lower complexity. Please see the detail in \cite{DAF-SC}.

\section{Differential Amplify-and-Forward Relaying in Time-Varying Rayleigh Fading Channels (three-node and multi-node)}
In these articles \cite{DAF-WCNC,DAF-ITVT}, we study a differential amplify-and-forward (D-AF) relaying (three-node and multi-node) over time-varying Rayleigh fading channels. Differential $M$PSK is used at the source to encode information. Relays forward the received signals to the destination after multiplying them with a fixed amplification factor. MRC technique using the conventional and also proposed combining weights in Section \ref{subsec:MRC} are utilized at the destination. Since, analysing the performance of the system using the fixed combining weights is too complicated (if not impossible), the performance of the system using optimum combining weights is analysed and the result is used as a lower bound for the actual system error performance. The pair-wise error probability (PEP) is obtained and used to approximate the average bit error probability (BEP) using nearest neighbour approximation. It is shown that an error floor exists at high signal-to-noise ratio (SNR) region, which is related to the auto-correlations of both the cascaded channel and the direct channel. Computer simulation are carried out for different number of relays and in various fading environments to support the analysis. The results illustrate that the proposed weights lead to a better performance than conventional weights in time-selective channels. Please see \cite{DAF-WCNC,DAF-ITVT} for details.


\section{Differential Dual-Hop Relaying over Time-Varying Rayleigh-Fading Channels}
In this part, we consider a special case of cooperative communication named dual-hop relay network. Dual-hop transmission has been studied in the literature as a technique to leverage coverage problems of many wireless applications such as 3GPP LTE, WiMAX, WLAN, Vehicle-to-Vehicle communication and wireless sensor networks \cite{coop-LTE,coop-WiMAX,coop-deploy,coop-dohler,coop-sensor}. Such a technique can be seen as a type of cooperative communication in which one node in the network helps another node to communicate with (for example) the base station when the direct link is very poor or out of coverage. The dual-hop system uses differential $M$-PSK modulation at the transmitter, AF strategy with a fixed gain at the relay, and non-coherent detection at the destination. We refer to this system as differential dual-hop (D-DH). Differential modulation with non-coherent detection is employed to avoid any channel estimation at the relay or destination. The non-coherent detection can be carried out over either two-symbol duration or multiple-symbol duration.
Despite multi-node D-AF \cite{DAF-WCNC,DAF-ITVT} that its exact BER cannot be achieved, with the two-symbol non-coherent detection, an exact bit error rate (BER) expression is obtained for the D-DH system. It is also shown that an error floor exists (at high transmit power), which is related to the auto-correlation of the cascaded channel. Since the two-symbol non-coherent detection does not perform well over fast time-varying channels, a near optimal
multiple-symbol differential sphere detection (MSDSD) scheme is developed. The MSDSD was first proposed for point-to-point systems in \cite{MSDSD-L} to reduce the complexity of multiple-symbol differential detection. In the context of relay networks, due to the complexity of the distribution of the received signal at the destination, the optimal decision rule of MSDSD cannot be easily obtained for the D-DH system under consideration. Instead, an alternative decision rule is proposed and its near optimal performance is illustrated with simulation results.






==> sections/gcw.tex <==
\chapter{Differential Amplify-and-Forward Relaying with Arbitrary Combining Weights}
\label{ch:gcw}

In Chapter~\ref{ch:mnode}, differential amplify-and-forward relaying system employing semi maximum-ratio-combining (semi-MRC) scheme was studied. In semi-MRC method, a set of fixed combining weights were determined based on the system parameters such as fading power and amplification factor. However, it would be useful to study D-AF relaying system with arbitrary combining weights. Specifically it is aimed to analyse and compare the performance of D-AF relaying system using semi-MRC weights and equal gain combining (EGC) method. In EGC method no priority given to the combined links and they are simply added together. Similar to selection combining scheme considered in Chapter~\ref{ch:sc} and Chapter~\ref{ch:sc_tv}, EGC method reduces the requirement to system parameters. 

The manuscript in this chapter lets the combining weights to be arbitrary. For a single-branch dual-hop relaying with direct link, the exact performance of the system in time-varying channels and general fading power is derived. The system performance using both semi-MRC wights and EGC weights are obtained, both theoretically and through simulations and compared with each other. The results show that, basically, there is no significant difference between the obtained results by both methods. This means that using EGC method, with no requirement to system parameters, does not sacrifice the system performance. From the results in this chapter and also Chapters~\ref{ch:sc},\ref{ch:sc_tv}, it can be concluded that the semi-MRC combining method can be replaced with either selection combining method or EGC method, depending on feasibility of implementation. It should be also mentioned that, due to complexity of analysis, the study in this chapter is limited to single-branch dual-hop relaying with direct link employing DBPSK encoding and decoding.

The result of our study has been reported in the following manuscript.

M. R. Avenid, Ha H. Nguyen, '' Differential amplify-and-forward relaying with arbitrary combining weights," \textit{submitted to ...}


==> sections/summary.tex <==
\chapter{Summary and Suggestions for Further Studies}
\label{ch:sum}

\section{Summary}
This thesis focussed mainly on developing and analysing differential encoding and decoding schemes for wireless amplify-and-forward (AF) relay networks. Specifically, the main contributions of this thesis are summarized as follows:

\begin{itemize}
\item A single-branch dual-hop relaying system without a direct link employing differential $M$-PSK and non-coherent detection was studied. First, two-symbol non-coherent detection was examined in time-varying channels and an exact BER expression was derived for the system performance. It was shown that the dependency of the BER to the channels auto-correlations causes a severe degradation and an error floor in the performance over rapid time-varying channels. Next, a near optimal multiple-symbol differential detection was designed and theoretically analysed. Simulation and theoretical results showed that the multiple-symbol differential detection is able to significantly improve the system performance in fast-fading channels.

\item
A multi-branch dual-hop relaying with a direct link employing differential $M$-PSK and two-symbol non-coherent detection was considered. A linear combiner with fixed combining weights was chosen to achieve the spatial diversity. The fixed combining weights were determined based on the second-order statistics of the channels. The performance of the system in practical time-varying channels was studied and a lower bound of the BER was derived. The theoretical and simulation results showed that the performance of the system degrades with channel variation and the existence of an error floor is inevitable.

\item
A single-branch dual-hop relaying system with a direct link employing selection combining at the destination was studied. Compared to the linear combiner, the selection combiner does not need any channel or system information. For the case of slow-fading channels, the exact BER and outage probability of this combiner using differential $M$-PSK were obtained. For the case of general time-varying channels (including both scenarios of slow-fading and fast-fading channels), an exact expression of the BER using DBPSK was derived. The simulation and theoretical results showed that the selection combiner does not suffer from system performance degradation, while it is simpler than the linear combiner.

\item
A multi-branch dual-hop relaying without a direct link employing differential distributed space-time coding strategy was considered. The performance of the system using two-symbol detection over time-varying channels was evaluated in terms of diversity. It was shown that two-symbol detection fails to perform well in fast-fading channels. A near optimal multiple-symbol differential detection was also developed. The simulation results showed the effectiveness of the multiple-symbol detection to improve the system performance in fast-fading channels.

\end{itemize}

\section{Future Studies}
The main objective of this thesis was to examine several important issues in cooperative communications using differential encoding and decoding. On the path toward achieving this objective, other issues came up and worthwhile to be investigated further. These issues are elaborated next.

\begin{itemize}

\item Selection combining was considered and analysed for a single-branch dual-hop relaying with a direct link. This combiner is attractive as it reduces the requirement of channels information while delivering similar performance to that of the linear combiner. For a multi-branch relaying system, more channel information would be needed for a linear combining. Although it appears difficult, it would be interesting to consider and analyse the performance of the selection combiner for multi-branch dual-hop relaying with/without a direct link as well. 


\item 
The performance analysis of multiple-symbol differential detection is important to reach a trade-off between the desired performance and the complexity of the decoding process. In this thesis, the performance of multiple-symbol differential detection for a single-branch dual-hop relaying without a direct link was derived. It would be then interesting to analytically evaluate the performance of multiple-symbol differential detection for multi-branch dual-hop relaying system with/without a direct link.

\item The developed multiple-symbol differential detection scheme requires the second-order statistics of all transmission links and also several other system parameters such as the noise variance and the amplification factor of the relays. In case that such information is not available nor accurate, multiple-symbol detection is not effective or near optimal. An alternative solution, yet challenging, is to develop a blind multiple-symbol differential detection that can deliver near optimal results.


\end{itemize}

